Stochastic Graph Neural Networks

Graph neural networks (GNNs) model nonlinear representations in graph data with applications in distributed agent coordination, control, and planning among others. Current GNN architectures assume ideal scenarios and ignore link fluctuations that occur due to environment, human factors, or external attacks. In these situations, the GNN fails to address its distributed task if the topological randomness is not considered accordingly. To overcome this issue, we put forth the stochastic graph neural network (SGNN) model: a GNN where the distributed graph convolution module accounts for the random network changes. Since stochasticity brings in a new learning paradigm, we conduct a statistical analysis on the SGNN output variance to identify conditions the learned filters should satisfy for achieving robust transference to perturbed scenarios, ultimately revealing the explicit impact of random link losses. We further develop a stochastic gradient descent (SGD) based learning process for the SGNN and derive conditions on the learning rate under which this learning process converges to a stationary point. Numerical results corroborate our theoretical findings and compare the benefits of SGNN robust transference with a conventional GNN that ignores graph perturbations during learning.

==> proofs.tex <==
%!TEX root = SGNNmain.tex

%%%%%%%%%%%%%%%%%%
%%% APPENDIX   %%%
%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Proposition 1} \label{pr:proposition1}

We need the following lemma, whose proof is in the supplementary material.

\begin{lemma} \label{lemmma3}
Consider the underlying graph $\ccalG$ with the shift operator $\bbS$ and let $\bbS_k$ be the shift operator of $k$th RES($\ccalG,p$) realization of $\bbS$, $\barbS=\mathbb{E}[\bbS_k]$ the expected shift operator, and $\bbD$ the diagonal degree matrix with $d_i$ the degree of node $i$. Then, it holds that
\begin{equation}\label{prlem33}
\mathbb{E}\left[ \bbS_k^2 \right] = 
\begin{cases}
\barbS^2 + p (1-p)\bbD,\! & \!\text{if } \bbS = \bbA, \\
\barbS^2 + 2 p (1-p)\bbS,\! & \!\text{if } \bbS = \bbL
\end{cases}
\end{equation}
with $\bbA$ the adjacency matrix and $\bbL$ the Laplacian matrix.  
\end{lemma}


\begin{proof}[Proof of Proposition \ref{proposition1}] 

Let $\bbu = \bbH(\bbS_{K:0})\bbx$ and $\barbu = \bbH(\barbS)\bbx$ be the output and the expected output of stochastic graph filter. Substituting the filter expression into the variance, we get\! \footnote{Throughout this proof, we will use the shorthand notation $\sum_{a,b,c = \alpha, \beta, \gamma}^{A, B, C} (\cdot)$ to denote $\sum_{a = \alpha}^A\sum_{b = \beta}^B\sum_{c = \gamma}^C (\cdot)$ to avoid overcrowded expressions. When the extremes of the sum ($\alpha, \beta, \gamma$ or $A, B, C$) are the same, we will write directly the respective value.}
\begin{gather} \label{eq:prop331}
\begin{split}
&{\rm var}[\bbu] = \mathbb{E} \left[ \tr \left( \bbu \bbu^{\rm H} - \bar{\bbu} \bar{\bbu}^{\rm H} \right) \right]\\
& = \sum_{k, \ell=0}^K h_k h_\ell \left( \mathbb{E} \left[ \tr \left( T(k,\ell) \right) \right] -  \mathbb{E} \left[ \tr \left( \bar{T}(k,\ell) \right) \right] \right)
\end{split}
\end{gather}
where $T(k,\ell)= \bbS_{k:0} \bbx \bbx^{\rm H} \bbS_{0:\ell}$ and $\bar{T}(k, \ell)= \bar{\bbS}^k  \bbx \bbx^{\top} \bar{\bbS}^\ell$. To further simplify notation, we denote with $\lceil k\ell \rceil = \max(k,\ell)$ and $\lfloor k\ell \rfloor = \min(k,\ell)$. Expression \eqref{eq:prop331} holds because of the linearity of the trace and expectation and the symmetry of the shift operators $\bbS_k$ and $\barbS$. Since $\bbS_k$ is a realization, we represent it as $\bbS_k = \barbS + \bbE_k$ where $\bbE_k$ is the deviation of $\bbS_k$ from the mean $\barbS$. Substituting this result into $T(k,\ell)$ and since $\mathbb{E}[\bbE_k] = \bb0$, we have
\begin{align}
\label{eq:prop33Ts1} &\mathbb{E}\left[ T(k,\ell)\right] = \mathbb{E}\left[ (\barbS + \bbE_k)\cdots \bbx \bbx^\top \cdots (\barbS + \bbE_\ell)\right]\\
&={\barbS}^{k}\bbx \bbx^\top {\barbS}^{\ell} \!+\! \mathbb{E}\!\left[\! \sum_{r=1}^{\lfloor k\ell \rfloor} \barbS^{k\!-\!r}\bbE_r \barbS^{r\!-\!1}\bbx \bbx^\top \barbS^{r\!-\!1}\bbE_r \barbS^{\ell\!-\!r}\!\right] \!+\! \mathbb{E}\!\left[\! \bbC_{k\ell}\!\right]. \nonumber 
\end{align}
The first term in \eqref{eq:prop33Ts1} yields from the maximum powers of $\barbS$ of the products; the second term captures all cross-products where we should note that for $k \ne \ell$ we have $\mathbb{E}\left[\bbE_k \bbE_\ell\right] = \mathbb{E}[\bbE_k]\mathbb{E}[\bbE_\ell] = \bb0$ due to independence and also the terms $r > \lfloor kl\rfloor$ are null due to the presence of a single expectation $\mathbb{E}[\bbE_r]$; the third term $\bbC_{k\ell}$ collects the sum of the remaining terms. By substituting $\tr \left( \mathbb{E}\left[ \bar{T}(k,\ell)\right] \right) = \tr \left( {\barbS}^{k}\bbx \bbx^\top {\barbS}^{\ell} \right)$ and \eqref{eq:prop33Ts1} into \eqref{eq:prop331}, we have
\begin{align} \label{eq:prop332}
&{\rm var}[\bbu] =\sum_{k=0}^K \sum_{\ell=0}^K h_k h_\ell \tr \left( \mathbb{E}\left[ \bbC_{k\ell}\right] \right)\\
& \! +\!\sum_{k=1}^K \sum_{\ell=1}^K h_k h_\ell \tr \left( \mathbb{E}\!\left[\! \sum_{r=1}^{\lfloor k\ell \rfloor} \barbS^{k-r}\bbE_r \barbS^{r\!-\!1}\bbx \bbx^\top \barbS^{r-1}\bbE_r \barbS^{\ell-r}\!\right] \right)\nonumber.
\end{align}
We now analyze the two terms in \eqref{eq:prop332} separately. For this analysis, we will need the inequality
\begin{gather} \label{eq:prop3ineq0}
\begin{split}
{\rm tr} (\bbA \bbB) \le \frac{\| \bbA + \bbA^\top \|_2}{2}{\rm tr}(\bbB) \le \| \bbA \|_2 {\rm tr}(\bbB)
\end{split}
\end{gather}
that holds for any square matrix $\bbA$ and positive semi-definite matrix $\bbB$ \cite{Wang1986}.

$\textbf{Second term.}$ By bringing the trace inside the expectation (due to their linearity) and leveraging the trace cyclic property $\tr(\bbA\bbB\bbC) = \tr(\bbC\bbA\bbB) = \tr(\bbB\bbC\bbA)$, we can write
\begin{align}
\label{eq:prop33} &\mathbb{E}\left[ \tr \left( \sum_{k,\ell=1}^K h_k h_\ell \sum_{r=1}^{\lfloor k\ell \rfloor} \barbS^{k-r}\bbE_r \barbS^{r-1}\bbx \bbx^\top \barbS^{r-1}\bbE_r \barbS^{\ell-r} \right) \right]\nonumber \\
& \!=\!\mathbb{E}\!\left[ \! \sum_{r=1}^K \tr\! \left( \!\sum_{k, \ell=r}^K \! h_k h_\ell \bbE_r \barbS^{k+\ell-2r}\bbE_r \barbS^{r-1}\bbx \bbx^\top\! \barbS^{r-1}\! \right)\!\right]\!.
\end{align}
Notice that in \eqref{eq:prop33} we also rearranged the terms to change the sum limits. Since both matrices $\sum_{k, \ell=r}^K h_k h_\ell \bbE_r \barbS^{k+\ell-2r}\bbE_r = \big(\sum_{k=r}^K h_k \barbS^{k-r}\bbE_r\big)^\top \big(\sum_{k=r}^K h_k \barbS^{k-r}\bbE_r\big)$ and $\barbS^{r-1}\bbx \bbx^\top \barbS^{r-1}$ are positive semi-definite, we can use the Cauchy-Schwarz inequality $\tr(\bbA \bbB) \le \tr(\bbA)\tr(\bbB)$ \cite{Zhang1999} to upper bound \eqref{eq:prop33} by
\begin{align}
\label{eq:prop34} \!\mathbb{E}\!\left[ \!\sum_{r\!=\!1}^K\! \sum_{k, \ell=r}^K \!h_k h_\ell \tr\! \left( \bbE_r \barbS^{k+\ell-2r}\bbE_r\! \right)\! \tr\! \left( \barbS^{r\!-\!1}\bbx \bbx^\top \barbS^{r\!-\!1} \!\right)\!\right]\!.
\end{align}

We now proceed by expressing the graph signal $\bbx$ in the frequency domain of the expected graph. Let $\barbS = \barbV\barbLambda\barbV^\top$ be the eigendecomposition of $\barbS$ with eigenvectors $\barbV = [\barbv_1,\ldots,\barbv_N]^\top$ and eigenvalues $\barbLambda = \text{diag}(\bar{\lambda}_1, \ldots, \bar{\lambda}_N)$. Substituting the graph Fourier expansion $\bbx = \sum_{i=1}^N \hat{x}_i \barbv_i$ into $\tr\! \left( \barbS^{r-1}\bbx \bbx^\top \barbS^{r-1} \right)$, we get
 \begin{gather}\label{eq:prop35}
\tr\! \left( \barbS^{r\!-\!1}\bbx \bbx^\top \barbS^{r\!-\!1} \right) \!=\! \sum_{i\!=\!1}^N\! \hat{x}_i^2 \bar{\lambda}_i^{2r\!-\!2} \tr\! \left(\! \barbv_i \barbv_i^\top\! \right) \!=\! \sum_{i\!=\!1}^N \hat{x}_i^2 \bar{\lambda}_i^{2r\!-\!2}
\end{gather}
where $\tr(\bbv_i\bbv_i^\top) = 1$ for $i=1,\ldots,N$ due to the orthonormality of eigenvectors. By substituting \eqref{eq:prop35} into \eqref{eq:prop34}, we get
\begin{align}
\label{eq:prop36} \!\sum_{i\!=\!1}^N \hat{x}_i^2 \mathbb{E}\!\left[ \! \sum_{r\!=\!1}^K \sum_{k, \ell=r}^K\! h_k h_\ell \bar{\lambda}_i^{2r-2} \tr\! \left( \bbE_r \barbS^{k+\ell-2r}\bbE_r \right)\!\right].
\end{align}
Using again the trace cyclic property to write $\tr(\bbE_r\barbS^{k+\ell-2}\bbE_r) = \tr(\barbS^{k+\ell-2}\bbE_r^2)$ and the linearity of the expectation, we have
\begin{align} \label{eq:prop37} 
& \sum_{i = 1}^N\hat{x}_i^2\! \sum_{r\!=\!1}^K\!\tr\! \left( \sum_{k, \ell=r}^K h_k h_\ell \bar{\lambda}_i^{2r-2} \barbS^{k+\ell-2r} \mathbb{E}\!\left[ \bbE_r^2\right] \right).
\end{align}
From Lemma \ref{lemmma3}, we have $\mathbb{E}\left[ \bbE_k^2 \right] =  \alpha p(1-p) \bbE$ with $\alpha = 1$ and $\bbE = \bbD$ if $\bbS = \bbA$ and $\alpha = 2$ and $\bbE = \bbS$ if $\bbS = \bbL$. By substituting this result into \eqref{eq:prop37} and using inequality \eqref{eq:prop3ineq0} since $\bbE$ is positive semi-definite, we have
\begin{align}
\label{eq:prop39}
& \sum_{i = 1}^N\hat{x}_i^2\! \sum_{r\!=\!1}^K\!\tr\! \left( \sum_{k, \ell=r}^K h_k h_\ell \bar{\lambda}_i^{2r-2} \barbS^{k+\ell-2r} \left( \alpha p(1-p) \bbE\right)\! \right)\\
& \le \!\alpha p(1-p)\sum_{i = 1}^N\hat{x}_i^2 \big\| \sum_{r\!=\!1}^K\! \sum_{k, \ell=r}^K\! h_k h_\ell \bar{\lambda}_i^{2r-2} \barbS^{k+\ell-2r} \big\|_2 \tr\! \left( \bbE \right) \nonumber
\end{align}
with $\tr\left( \bbE \right)=\sum_{i=1}^N d_i =2M$ and $M$ the number of edges. 

At this point, we proceed to upper bound the filter matrix norm in \eqref{eq:prop39}. A standard procedure to bound the spectral norm of a matrix $\bbA$, is to upper bound the norm of $\|\bbA\bba\|_2$ as $\|\bbA\bba\|_2 \le A \|\bba\|_2$ for any vector $\bba$ \cite{Meyer2000}. In this instance, $A$ is the upper bound for the norm of $\bbA$. Following this rationale, we consider the GFT expansion of a vector $\bba$ on the expected graph $\bba = \sum_{j=1}^N \hat{a}_j \barbv_j$ where $\{ \barbv_j \}_{j=1}^N$ are orthonormal. Then, we have
\begin{align}
\label{eq:prop310} & \!\big\| \!\sum_{r\!=\!1}^K\!\! \sum_{k, \ell\!=\!r}^K\! h_k\! h_\ell\! \bar{\lambda}_i^{2r\!-\!2}\! \barbS^{k\!+\!\ell\!-\!2r}\! \bba \big\|_2^2 \!\!=\!\! \sum_{j\!=\!1}^N\!\! \hat{a}_j^2 \big|\! \sum_{r\!=\!1}^K\!\! \sum_{k, \ell\!=\!r}^K\! h_k\! h_\ell\! \bar{\lambda}_i^{2r\!-\!2}\! \bar{\lambda}_j^{k\!+\!\ell\!-\!2r}\big|^2\!\!.
\end{align}
Consider now the expression inside the absolute value in \eqref{eq:prop310}. This expression is linked to the partial derivative of the generalized frequency response $h(\bblambda)$ in \eqref{eq:h2}. To detail this, we introduce the first-order partial derivative of the generalized frequency response $h(\bblambda)$ w.r.t. the $r$th entry $\lambda_r$ of $\bblambda$
\begin{align}
\label{eq:prop31051} 
\frac{\partial h(\bblambda)}{\partial \lambda_r} \!=\! \sum_{k=r}^K h_k \lambda_{K:(r+1)} \lambda_{(r-1):1},\! ~\forall~r\!=\!1,\!\ldots,\!K
\end{align}
where $\lambda_{K:(r+1)} = \lambda_K \cdots \lambda_{r+1}$ and $\lambda_{(r-1):1}=\lambda_{r-1}\cdots \lambda_1$. Let us then consider $K$ specific eigenvalue vectors of dimensions $K\times 1$: $\barblambda_{ij}^1 = [\bar{\lambda}_j, ..., \bar{\lambda}_j]^\top$, $\barblambda_{ij}^2 = [\bar{\lambda}_i, \bar{\lambda}_j, \ldots, \bar{\lambda}_j]^\top$, $\ldots$ , $\barblambda_{ij}^K = [\bar{\lambda}_i, ...,\bar{\lambda}_i, \bar{\lambda}_j]^\top$ for two eigenvalues $\bar{\lambda}_i$ and $\bar{\lambda}_j$ of $\barbS$, and their respective generalized frequency responses $\{ h(\barblambda_{ij}^1), \ldots, h(\barblambda_{ij}^K) \}$\!\!\! \footnote{The generalized frequency response $h(\bblambda)$ in \eqref{eq:frere1} is an analytic function of the vector variable $\bblambda = [\lambda_1, \ldots, \lambda_K]^\top$ such that $\bblambda$ can take any value.} [cf. \eqref{eq:frere1}]. The $r$th first-order partial derivative $\partial h(\bblambda)/\partial \lambda_r$ of the generalized frequency response instantiated on $\barblambda_{ij}^r$ is
\begin{align}
\label{eq:prop3105} 
\frac{\partial h(\barblambda_{ij}^r)}{\partial \lambda_r} = \sum_{k=r}^K h_k \bar{\lambda}_{i}^{r-1} \bar{\lambda}_j^{k-r},\! ~\forall~r\!=\!1,\!\ldots,\!K.
\end{align}
We then observe the expression inside the absolute value in \eqref{eq:prop310} can be represented as the sum of $K$ first-order partial derivatives; i.e., we can write it in the compact form
\begin{align}
\label{eq:prop311} &\sum_{r\!=\!1}^K\! \sum_{k, \ell=r}^K\! h_k h_\ell \bar{\lambda}_i^{2r-2} \bar{\lambda}_j^{k+\ell-2r} =  \sum_{r\!=\!1}^K \left( \frac{\partial h(\barblambda_{jr})}{\partial\lambda_{r}} \right)^2.
\end{align}
From Assumption \ref{as:4}, the generalized frequency responses are Lipschitz with constant $C_g$. Thus we can upper bound \eqref{eq:prop311} as
\begin{align}
\label{eq:prop3115} & \big| \sum_{r\!=\!1}^K\! \sum_{k,\ell=r}^K\! h_k h_\ell \bar{\lambda}_i^{2r-2} \bar{\lambda}_j^{k+\ell-2r}\big|^2  \le K^2 C_g^4
\end{align}
which implies the norm of the filter matrix in \eqref{eq:prop310} is upper bounded by $KC_g^2$.

By substituting this norm bound into \eqref{eq:prop310} and altogether into \eqref{eq:prop33}, we have
\begin{align}
\label{eq:prop312} &\mathbb{E}\left[ \sum_{k, \ell=1}^K h_k h_\ell \sum_{r=1}^{\lfloor k\ell \rfloor} \tr \left( \barbS^{k-r}\bbE_r \barbS^{r-1}\bbx \bbx^\top \barbS^{r-1}\bbE_r \barbS^{\ell-r} \right) \right]\nonumber \\
& \!\le\! 2\alpha MKC_g^2 \!\sum_{i\!=\!1}^N \!\hat{x}_i^2 p(1\!-\!p) \!=\! 2\alpha MKC_g^2\| \bbx \|^2_2 p(1\!-\!p).
\end{align}

$\textbf{First term.}$ Matrix $\bbC_{k\ell}$ comprises the sum of the remaining expansion terms. Each of these terms is a quadratic form in the error matrices $\bbE_k$, $\bbE_\ell$ with $k \neq l$; i.e., it is of the form $f_1(\barbS, h_k)\bbE_k f_2(\barbS, h_k)\bbE_kf_3(\barbS, h_k)\bbE_\ell f_4(\barbS, h_k)\bbE_\ell$ for some functions $f_1(\cdot), ..., f_4(\cdot)$ that depend on the expected shift operator and filter coefficients. Each of these double-quadratic terms can be bounded by a factor containing at least two terms $\tr\left(\mathbb{E}[\bbE_{k_1}^2]\right)$ and $\tr\left(\mathbb{E}[\bbE_{k_2}^2]\right)$. Since the frequency response $h(\lambda)$ is bounded from Assumption \ref{as:3}, also the coefficients $\{ h_k \}_{k=0}^K$ are bounded. Further since $\| \barbS \|_2$ is bounded and $\mathbb{E}[\bbE_{k}^2] = \alpha p(1-p)\bbE$ from Lemma \ref{lemmma3}, we can write the first term in \eqref{eq:prop33Ts1} as
\begin{gather} \label{eq:prop3125}
\begin{split}
 \mathbb{E} \left[\sum_{k, \ell=0}^K h_k h_\ell \bbC_{k\ell} \right] = \ccalO(p^2(1-p)^2)\|\bbx\|_2^2.
\end{split}
\end{gather}

Finally, substituting the results for the first term \eqref{eq:prop3125} and second term \eqref{eq:prop312} into \eqref{eq:prop33Ts1}, we have the variance bound
\begin{gather} \label{eq:prop3313}
\begin{split}
& {\rm var} \left[ \bbu_s \right] \le 2 \alpha M K C_g^2 \| \bbx \|_2^2 p(1-p) + \ccalO(p^2 (1-p)^2)
\end{split}
\end{gather}
completing the proof.
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Theorem 1} \label{pr:theorem1}

In the proof, we need the following lemma with the proof in the supplementary material that shows the bound on the filter output.

\begin{lemma} \label{lemmma1}
Consider the graph filter $\bbH(\bbS)$ [cf. \eqref{eq:sgf2} for $p = 1$] with coefficients $\{h_k\}_{k=0}^K$ and let $\bbS$ be the graph shift operator. Let the frequency response \eqref{eq:frere1} satisfy Assumption \ref{as:3} with constant $C_U$. Then, the norm of the graph filter is upper bounded as
\begin{equation} \label{eq:lemmmamain}
\begin{split}
\| \bbH(\bbS) \|_2 \le C_U.
\end{split}
\end{equation}
\end{lemma}

\begin{proof}[Proof of Theorem \ref{theorem1}]
From the SGNN definition in \eqref{eq.sgnn} and Assumption \ref{assumption3}, the variance can be upper bounded as
\begin{equation} \label{eq:thm41}
\begin{split}
& \!{\rm var} \!\left[ \bbPhi(\bbx;\bbS_{P:1},\!\ccalH) \right] \!\!=\! {\rm var}\!\! \left[\! \sigma\!\!\left(\!\sum_{f\!=\!1}^{F}\! \bbu^f_{L-1}\!\!\right)\! \!\right] \!\!\!\le\!  {\rm var}\! \!\left[ \!\sum_{f\!=\!1}^{F}\! \bbu^f_{L\!-\!1}\!\! \right]\!
\end{split}
\end{equation}
where ${\rm var}[\cdot]$ is defined in \eqref{eq:var0}. By exploiting the relation between the trace of covariance matrix and the variance, we can rewrite \eqref{eq:thm41} as
\begin{align} \label{eq:thm42}
{\rm var}\! \left[ \!\sum_{f=1}^{F}\! \bbu^f_{L-1}\! \right] &= \!\tr\! \left( \mathbb{E}\! \left[\!\big(\! \sum_{f=1}^{F}\! \bbu^f_{L-1}\!\big) \big(\! \sum_{f=1}^{F}\! \bbu^f_{L-1}\!\big)^\top\! \right]\! \right. \nonumber\\
& \left. - \mathbb{E}\!\!\left[\!\sum_{f=1}^{F}\! \bbu^f_{L-1}\! \right]\!\! \mathbb{E}\!\!\left[\!\sum_{f=1}^{F}\! \bbu^f_{L-1}\! \right]^\top\! \right)\!. 
\end{align}
Denote $\bbu_{L-1}^f = \bbH_{L}^{f} \bbx^f_{L-1}$ and $\barbu_{L-1}^f=\barbH_L^f \bbx_{L-1}^f$ as concise notations of stochastic graph filter output $\bbH_{L}^f(\bbS_{K:0}) \bbx^f_{L-1}$ and expected graph filter output $\mathbb{E}\left[ \bbH_{L}^f(\bbS_{K:1}) \right]\bbx^f_{L-1}=\bbH_{L}^f(\barbS) \bbx^f_{L-1}$. By expanding \eqref{eq:thm42}, we get
 \begin{align} \label{eq:thm43}
& {\rm var}\! \left[ \!\sum_{f=1}^{F}\! \bbu^f_{L-1}\! \right] \!= \!\sum_{f\!=\!1}^{F}\! \sum_{g\!=\!1}^{F}\tr\! \left(\!  \mathbb{E} \!\left[ \!\bbH_{L}^{f} \bbx^f_{L-1}\! \left( \bbH_{L}^{g} \bbx^{g}_{L-1} \right)^\top \!\right.  \right] \nonumber\\
& \quad \quad \quad \quad \quad \quad \left.  - \mathbb{E}\left[ \bbH_{L}^{f} \bbx^f_{L-1} \right] \mathbb{E} \left[ \bbH_{L}^{g} \bbx^{g}_{L-1} \right]^\top \right).
\end{align}
By adding and subtracting $\barbH_{L}^{f} \bbx^f_{L-1} \left( \barbH_{L}^{g} \bbx^{g}_{L-1}\right)^\top$ inside the first expectation, \eqref{eq:thm43} becomes
 \begin{align} \label{eq:thm44}
& \! \sum_{f\!=\!1}^{F}\! \sum_{g\!=\!1}^{F}\!\tr\! \left(\! \mathbb{E} \!\left[ \!\bbH_{L}^{f}\! \bbx^f_{L-1}\! \left( \bbH_{L}^{g}\! \bbx^{g}_{L-1} \right)^\top \!-\!\barbH_{L}^{f}\! \bbx^f_{L-1}\! \left( \barbH_{L}^{g}\! \bbx^{g}_{L-1}\right)^\top \!\right. \right] \nonumber\\
&  \!\!+\!\mathbb{E}\!\left[ \barbH_{L}^{f}\! \bbx^f_{L\!-\!1}\! \left( \barbH_{L}^{g}\! \bbx^{g}_{L\!-\!1}\right)^\top \right]\! \left.\!- \mathbb{E}\!\left[ \bbH_{L}^{f} \bbx^f_{L\!-\!1} \!\right]\! \mathbb{E}\! \left[ \bbH_{L}^{g} \bbx^{g}_{L\!-\!1} \right]^\top\! \right)\!.\!
\end{align}
Expression \eqref{eq:thm44} is composed of two group of terms shown there in the two separate lines. 

\textbf{First term.} For the first term, when $f \ne g$ such that filters $\bbH_{L}^{f}(\bbS_{K:0})$ and $\bbH_{L}^{g}(\bbS_{K:0})$ are independent, we have
 \begin{equation} \label{eq:thm455}
\begin{split}
& \!\tr\! \left(\! \mathbb{E} \!\left[ \!\bbH_{L}^{f}\! \bbx^f_{L\!-\!1}\! \left( \bbH_{L}^{g}\! \bbx^{g}_{L\!-\!1} \right)^\top \!-\!\barbH_{L}^{f}\! \bbx^f_{L-1}\! \left( \barbH_{L}^{g} \bbx^{g}_{L\!-\!1}\right)^\top \right] \right)\!=\! 0.
\end{split}
\end{equation}
We then use \eqref{eq:thm455} to derive the upper bound
 \begin{align} \label{eq:thm45}
& \!\sum_{f\!=\!1}^{F}\! \sum_{g\!=\!1}^{F}\!\tr\! \left(\! \mathbb{E} \!\left[ \!\bbH_{L}^{f}\! \bbx^f_{L-1}\! \left(\! \bbH_{L}^{g}\! \bbx^{g}_{L\!-\!1} \!\right)^\top \!-\!\barbH_{L}^{f}\! \bbx^f_{L-1}\! \left( \barbH_{L}^{g}\! \bbx^{g}_{L-1}\right)^\top \right]\! \right)\!\nonumber\\
& = \!\sum_{f\!=\!1}^{F}\!\tr\! \left( \mathbb{E} \!\left[ \!\bbH_{L}^{f}\! \bbx^f_{L\!-\!1}\! \left(\! \bbH_{L}^{f}\! \bbx^{f}_{L\!-\!1} \!\right)^\top \!-\!\barbH_{L}^{f}\! \bbx^f_{L\!-\!1}\! \left( \!\barbH_{L}^{f}\! \bbx^{f}_{L\!-\!1}\!\right)^\top \!\right]\! \right)\! \nonumber\\
& \le \Delta \sum_{f=1}^{F}\! \mathbb{E}\left[ \| \bbx^f_{L\!-\!1} \|_2^2 \right] p(1\!-\!p) \!+\! \mathcal{O}(p^2 (1\!-\!p)^2)
\end{align}
where $\Delta = 2\alpha M\! K\! C_g^2$ and the last inequality holds from Proposition \ref{proposition1}. For the norm of $\bbx_{L-1}^f$, we observe that
\begin{equation}\label{eq:thm456}
\begin{split}
\mathbb{E}\!\!\left[ \| \bbx^f_{L\!-\!1} \|_2^2 \right] \!=\! \mathbb{E}\!\!\left[ \Big\| \sigma \!\!\left( \sum_{g=1}^F \bbu_{L\!-\!2}^{fg} \right) \!\Big\|_2^2 \right] \!\le\!C_\sigma^2 F\! \sum_{g=1}^F\! \mathbb{E}\!\left[ \left\| \bbu_{L\!-\!2}^{fg} \right\|_2^2 \right]
\end{split}
\end{equation}
where Assumption \ref{assumption3} and the triangle inequality are used in the last inequality. By further representing $\big\| \bbu_{L\!-\!2}^{fg} \big\|_2^2$ with the trace $\tr (\bbu_{L-2}^{fg} (\bbu_{L-2}^{fg})^\top)$ and expanding the latter as in \eqref{eq:prop33Ts1}, we have
\begin{align}
\label{eq:thm458} &\!\!\mathbb{E}\!\left[\!\bbu_{L-2}^{fg} (\bbu_{L-2}^{fg})^\top\!\right]\! \!=\!\!\! \sum_{k,\ell=0}^K \!\!h_{k(L-2)}^{fg}h_{\ell(L-2)}^{fg}{\barbS}^{k}\mathbb{E}\!\left[\bbX_{L-2}^g\right] {\barbS}^{\ell}\\
&\!\!\!\!\!+\!\!\!\!\!\sum_{k,\ell=0}^K\!\!\!\! h_{k(L\!-\!2)}^{fg}\!h_{\ell(L\!-\!2)}^{fg}\!\!\! \left(\!\! \mathbb{E}\!\!\left[\! \sum_{r=\!1}^{\lfloor\! k\ell\! \rfloor}\!\! \barbS^{k\!-\!r}\!\bbE_r\! \barbS^{r\!-\!1}\!\bbX_{L\!-\!2}^g \barbS^{r\!-\!1}\!\bbE_r\! \barbS^{\ell\!-\!r}\!\!\right]\!\! \!+\!\! \mathbb{E}\!\left[ \bbC_{k\ell}\right]\!\!\right) \nonumber 
\end{align}
with $\bbX_{L-2}^g = \bbx_{L-2}^g (\!\bbx_{L-2}^g)^\top$. For the first term, by using the cyclic property of trace and the inequality \eqref{eq:prop3ineq0}, we can bound it as
\begin{align} \label{eq:thm459}
&\tr \left( \sum_{k,\ell=0}^K\! h_{k(L\!-\!2)}^{fg}h_{\ell(L\!-\!2)}^{fg}{\barbS}^{k}\mathbb{E}\!\left[\bbX_{L-2}^g\right] {\barbS}^{\ell}\right)\nonumber\\
& \le \| \sum_{k,\ell=0}^K \!h_{k(L-2)}^{fg}h_{\ell(L-2)}^{fg} \bar{\bbS}^{k+\ell} \|_2 \tr \left( \mathbb{E}\!\left[\bbX_{L-2}^g\right] \right)  \\
& = \| \barbH_{L-2}^{fg} \barbH_{L-2}^{fg} \|_2 \tr \left( \mathbb{E}\!\left[\bbX_{L-2}^g \right]\right) \le C_U^2 \mathbb{E}\left[\|\bbx_{L-2}^{g} \|^2_2\right]\nonumber
\end{align}
where in the last inequality we used Lemma \ref{lemmma1} and $\tr \left( \mathbb{E}\left[\bbX_{L-2}^g \right]\right) = \mathbb{E}\left[\|\bbx_{L-2}^{g} \|^2_2\right]$. For the second term and the third term, we use the result \eqref{eq:prop312} and \eqref{eq:prop3125} to write
\begin{align}
\label{eq:thm4510} &\sum_{k,\ell\!=\!0}^K\!\!\! h_{k(L\!-\!2)}^{fg}\!h_{\ell(L\!-\!2)}^{fg} \!\tr\!\! \left(\!\! \mathbb{E}\!\!\left[\! \sum_{r\!=\!1}^{\lfloor\! k\ell\! \rfloor}\! \barbS^{k\!-\!r}\bbE_r\! \barbS^{r\!-\!1}\!\bbX_{L\!-\!2}^g \barbS^{r\!-\!1}\bbE_r\! \barbS^{\ell\!-\!r}\!\!+\!\! \bbC_{k\ell}\!\right]\!\!\right)\nonumber\\
& \le \ccalO(p(1-p)).
\end{align}
By substituting \eqref{eq:thm459} and \eqref{eq:thm4510} into \eqref{eq:thm458} and the latter into \eqref{eq:thm456}, we get
\begin{equation}\label{eq:thm4511}
\begin{split}
\mathbb{E}\!\!\left[ \| \bbx^f_{L\!-\!1} \|_2^2 \right] \!\le\!  C_\sigma^2 C_U^2 F \sum_{g=1}^F \mathbb{E}\!\!\left[ \left\| \bbx_{L\!-\!2}^{g} \right\|_2^2 \right] \!+\! \ccalO(p(1-p)).
\end{split}
\end{equation}
Solving recursion \eqref{eq:thm4511} with the initial condition $\| \bbx_0^1 \|_2^2 = \| \bbx \|_2^2$ yields
\begin{equation}\label{eq:thm4512}
\begin{split}
& \mathbb{E}[ \| \bbx_{L-1}^f \|_2^2]\! \le\!  C_\sigma^{2L-2}C_U^{2L\!-2}F^{2L\!-4}  \| \bbx \|_2^2 \!+\! \ccalO(p(1-p)).
\end{split}
\end{equation}
By substituting \eqref{eq:thm4512} into \eqref{eq:thm45}, we bound \eqref{eq:thm45} by 
\begin{equation} \label{eq:thm46}
\begin{split}
\Delta F^{2L-3} C_\sigma^{2L-2}C_U^{2L-2} \| \bbx \|_2^2 p(1-p)  + \mathcal{O}(p^2(1-p)^2).
\end{split}
\end{equation}

\textbf{Second term.} For the second term in \eqref{eq:thm44}, we have\!\! \footnote{Likewise \eqref{eq:var0}, we use the notation ${\rm cov}[\bbx, \bby] = \sum_{i=1}^N {\rm cov}[[\bbx]_i, [\bby]_i]$ for any two random vectors $\bbx$ and $\bby$.}
 \begin{align} \label{eq:thm47}
& \! \sum_{f\!=\!1}^{F}\! \sum_{g\!=\!1}^{F}\! \tr\!\left(\! \mathbb{E} \! \left[ \!\barbH_{L}^{f}\!\bbx^f_{L\!-\!1}\! \left( \!\barbH_{L}^{g}\!\bbx^{g}_{L\!-\!1}\!\right)^\top \! \right] \! -\! \mathbb{E}\!\left[\! \barbH_{L}^{f}\!\bbx^f_{L\!-\!1}\! \right]\! \mathbb{E} \!\left[\! \barbH_{L}^{g}\!\bbx^{g}_{L\!-\!1}\! \right]^\top \right) \nonumber\\
& \!= \! \sum_{f=1}^{F} \! {\rm var} \! \left[ \!\barbH_{L}^{f}\!\bbx^f_{L-1} \!\right] \!+\! \sum_{f \ne g}^{F} \! {\rm cov} \! \left[ \! \barbH_{L}^{f}\!\bbx^f_{L-1}, \barbH_{L}^{g}\!\bbx^{g}_{L\!-\!1} \right].
\end{align}
By using the property of covariance \cite{Chandler1987}
\begin{equation} \label{eq:thm48}
\begin{split}
 {\rm cov}[x,y] \le \sqrt{{\rm var}[x]} \sqrt{{\rm var}[y]} \le \frac{{\rm var}[x]+{\rm var}[y]}{2} 
\end{split}
\end{equation}
for two random variables $x$ and $y$, we can bound \eqref{eq:thm47} by
 \begin{align} \label{eq:thm485}
&F \sum_{f=1}^{F} \! {\rm var} \! \left[ \!\barbH_{L}^{f}\!\bbx^f_{L-1} \!\right] =\! F\sum_{f=1}^{F} \tr\left( \barbH_{L}^{f} \barbH_{L}^{f}\bbSigma_{L-1}^f \right)
\end{align}
where $\bbSigma_{L-1}^f = \mathbb{E} \! \left[ \left( \!\bbx^f_{L\!-\!1}\! -\! \mathbb{E}\!\left[\! \bbx^f_{L\!-\!1}\! \right] \right) \left( \!\bbx^f_{L\!-\!1}\! -\! \mathbb{E}\!\left[\! \bbx^f_{L\!-\!1}\! \right] \right)^\top \right]$ is positive semi-definite matrix for all $f=1,\ldots,F$ and $\barbH_{L}^{f}\! \barbH_{L}^{f}$ is square. We then refer to inequality \eqref{eq:prop3ineq0} to bound \eqref{eq:thm485} as
 \begin{align} \label{eq:thm49}
&\| \barbH_{L}^{g} \|_2^2 F \!\sum_{f\!=\!1}^{F}\! \tr\!\left( \bbSigma_{L-1}^f  \right)  \le C_U^2 F \sum_{g=1}^{F} {\rm var} \left[ \bbx^f_{L-1} \right]
\end{align}
where the last inequality is due to Lemma \ref{lemmma1}. By substituting bounds \eqref{eq:thm46} and \eqref{eq:thm49} into \eqref{eq:thm44} and then altogether into \eqref{eq:thm42}, we observe a recursion where the variance of $\ell$th layer output depends on the variance of $(\ell-1)$th layer output as well as the bound in \eqref{eq:thm46}. Therefore, we have
\begin{align} \label{eq:thm410}
&{\rm var}[\bbx_L]\!:=\!{\rm var} \left[ \bbPhi(\bbx;\bbS_{P:1},\!\ccalH) \right] \! \le\! C_U^2 F \!\sum_{f=1}^{F}\! {\rm var} \left[ \bbx^f_{L-1} \right]  \\
& + \Delta F^{2L-3} C_\sigma^{2L-2}C_U^{2L-2} \| \bbx \|_2^2 p(1-p)  + \mathcal{O}(p^2(1-p)^2).\nonumber
\end{align}

\textbf{Unrolling.} By expanding this recursion until the input layer, we have
\begin{align} \label{eq:thm411}
& {\rm var}\!\! \left[ \bbPhi(\bbx;\bbS_{P:1},\!\ccalH) \right] \!\!\le\!\! \Delta\!\! \sum_{\ell\!=\!2}^L \!\!F^{2L\!-\!3} C_\sigma^{2\ell\!-\!2} C_U^{2L\!-\!2} \| \bbx \|_2^2 p(\!1\!-\!p\!) \\
& \!\!+\!\! F^{2L\!-\!4} C_U^{2L\!-\!2}\!\! \left(\! \sum_{f\!=\!1}^{F} \!\!{\rm var}\! \left[ \bbx^f_1 \right] \!\!+ \!\!\!\sum_{f\ne g}^{F} \!\!{\rm cov}\! \left[ \!\bbx^f_1, \bbx^g_1 \!\right]\!\! \right)\! \!\!+\! \mathcal{O}\left(p^2(1\!-\!p)^2\right)\nonumber
\end{align}
where the first term in \eqref{eq:thm411} is the accumulated sum of all second terms in \eqref{eq:thm410} during the recursion. Since $\bbx_1^f = \bbH_{1}^f \bbx$ and $\bbx_1^g = \bbH_{1}^g \bbx$ and $\bbH_{1}^f$ and $\bbH_{1}^g$ are independent if $f \ne g$, we have $\sum_{f\ne g}^{F} \!{\rm cov}\!\! \left[ \bbx^f_1, \bbx^g_1 \right]=0$. Therefore, \eqref{eq:thm411} becomes
\begin{align} \label{eq:thm412}
& {\rm var} \left[ \bbPhi(\bbx;\bbS_{P:1},\!\ccalH) \right] \le \ccalO(p^2(1\!-\!p)^2) \\ 
& ~~~~~~~+  2\alpha M \sum_{\ell=1}^L F^{2L-3} C_\sigma^{2\ell-2} C_U^{2L-2}K C_g^2 \| \bbx \|_2^2 p(1-p) \nonumber.
\end{align}
This completes the proof.
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Proof of Theorem 2} \label{pr:theorem2}

\begin{proof}
From the Taylor expansion of $\mathbb{E} \left[ \bar{C}(\ccalH_{t+1}) \right]$ at $\ccalH_t$, we have
\begin{align} \label{eq:prthm11}
&\mathbb{E}\!\left[ \bar{C}(\ccalH_{t\!+\!1})\right] \!\!=\! \mathbb{E}\!\left[ \bar{C}(\ccalH_{t}) \right. \!\!+\!\! \nabla_\ccalH \bar{C}(\ccalH_{t})^\top \!\left(\ccalH_{t+1}-\ccalH_t\right) \\
&~~~~~~~~~~~~~~+\!\frac{1}{2}\left( \ccalH_{t\!+\!1}\!-\!\ccalH_t\right)^\top \nabla^2_\ccalH \bar{C} (\tilde{\ccalH}_{t}) \left( \ccalH_{t\!+\!1}-\ccalH_t\right) \big]\! \nonumber
\end{align}
where $\tilde{\ccalH}_{t}$ is in the line segment joining $\ccalH_{t+1}$ and $\ccalH_{t}$, and we substituted $\tilde{\ccalH}_{t}$ in the Hessian term $\nabla^2_\ccalH \bar{C} (\tilde{\ccalH}_{t})$ of \eqref{eq:prthm11} for the series truncation. Since for any vector $\bba$ and matrix $\bbA$, we have the inequality $\bba^\top \bbA \bba \le \lambda_{\max}(\bbA) \| \bbx \|_2^2$ where $\lambda_{\max}(\bbA)$ is the largest eigenvalue of $\bbA$. With this result and the Lipschitz continuity $\| \nabla^2_\ccalH \bar{C} (\tilde{\ccalH}_{t}) \|_2 \le C_L$ in Assumption \ref{as:1}, we get
\begin{align} \label{eq:prthm12}
&\mathbb{E}\!\!\left[ \bar{C}(\!\ccalH_{t+1}\!)\right] \\
&\le \mathbb{E}\big[ \bar{C}(\!\ccalH_{t}\!)\! +\! \nabla_\ccalH \bar{C}(\!\ccalH_{t}\!)^\top\! \!\left(\! \ccalH_{t\!+\!1}\!-\!\ccalH_t\!\right) \!+\! \frac{C_L}{2}\! \| \ccalH_{t\!+\!1}\!-\!\ccalH_t \|_2^2\big]\!. \nonumber
\end{align}
By substituting the SGNN update rule $\ccalH_{t+1} = \ccalH_t - \alpha_t \nabla_\ccalH C(\bbS_{P:1}, \ccalH_t)$ with random cost realization, we get
\begin{align} \label{eq:prthm125}
\mathbb{E}\!\left[ \bar{C}(\ccalH_{t\!+\!1})\right]\! &\le \!\mathbb{E}\!\big[ \bar{C}(\ccalH_{t}) + \!\frac{\alpha_t^2 C_L}{2}\! \| \nabla_\ccalH C(\bbS_{P:1}, \ccalH_t) \|_2^2 \nonumber\\
&- \alpha_t \nabla_\ccalH \bar{C}(\ccalH_t)^\top \nabla_\ccalH C(\bbS_{P:1}, \ccalH_t) \big].   
\end{align}
Exploiting the linearity of expectation and the identity $\mathbb{E}[\nabla_\ccalH C(\bbS_{P:1},\! \ccalH_t)]=\mathbb{E}[\nabla_\ccalH \bar{C}(\ccalH_t)]$, we can write \eqref{eq:prthm125} as
\begin{align} \label{eq:prthm13}
\mathbb{E}\left[ \bar{C}( \ccalH_{t+1})\right] &\le \mathbb{E}\big[ \bar{C}( \ccalH_t) ] \!-\! \alpha_t \mathbb{E}\big[\| \nabla_\ccalH \bar{C}(\ccalH_t) \|_2^2\big] \\
&\!+\! \frac{\alpha_t^2 C_L}{2} \mathbb{E} [\| \nabla_\ccalH C(\bbS_{P:1}, \ccalH_t) \|_2^2\big].   \nonumber  
\end{align}
Subsequently, using the gradient bound in Assumption \ref{as:2}, we can upper bound the third term of \eqref{eq:prthm13} as
\begin{equation} \label{eq:prthm14}
\begin{split}
\frac{\alpha_t^2 C_L}{2} \mathbb{E} [\| \nabla_\ccalH C(\bbS_{P:1},\! \ccalH_t) \|_2^2] \le \frac{\alpha_t^2 C_L C_B^2}{2}.
\end{split}
\end{equation}
Since $\| \nabla_\ccalH \bar{C}(\ccalH_t) \|^2_2 \le \epsilon$ is the convergence criterion for non-convex problems, we focus on the second term in \eqref{eq:prthm13}. We first move it to the left side, and then move $\mathbb{E}\left[ \bar{C}(\ccalH_{t+1})\right]$ on the right side, and finally define the difference between two successive costs as
\begin{align} \label{eq:prthm145}
\Delta \bar{C}_{t:t+1} =\! \bar{C}( \ccalH_t) \!-\! \bar{C}(\ccalH_{t+1}).
\end{align}
With these arithmetic steps, we can rewrite \eqref{eq:prthm13} as
\begin{equation} \label{eq:prthm15}
\begin{split}
\mathbb{E}[\| \nabla_\ccalH \bar{C}(\ccalH_t) \|_2^2] \le \frac{1}{\alpha_t} \mathbb{E}[ \Delta \bar{C}_{t:t+1} ]+ \frac{\alpha_t C_L C_B^2}{2}.
\end{split}
\end{equation}
By considering a constant step $\alpha_t = \alpha$ and summing up all terms in \eqref{eq:prthm15} -- recall \eqref{eq:prthm15} should hold for all $t = 0, \cdots, T-1$ -- we get
\begin{equation}\label{eq:prthm155}
\begin{split}
\sum_{t=0}^{T-1} \!\mathbb{E}[\| \nabla_\ccalH \bar{C}(\ccalH_t) \|^2] \le \frac{1}{\alpha} \mathbb{E}[ \Delta \bar{C}_{0:T} ]\!+\! \frac{ \alpha T C_L C_B^2}{2}.
\end{split}
\end{equation}
For the optimal tensor $\ccalH^*$, we have $\bar{C} (\ccalH^*)\! \le\! \bar{C} ( \ccalH_{T})$. By substituting this result into $\Delta \bar{C}_{0:T}$, we bound \eqref{eq:prthm155} as
\begin{align} \label{eq:prthm16}
&\min_t \mathbb{E}[\| \nabla_\ccalH \bar{C}(\ccalH_t) \|^2] \le \frac{1}{T}\! \sum_{t=0}^{T-1}\! \mathbb{E}[\| \nabla_\ccalH \bar{C}(\ccalH_t) \|^2] \nonumber \\
& \le \frac{1}{T \alpha} \left( \bar{C} (\ccalH_0) - \bar{C} (\ccalH^*) \right)+ \frac{ \alpha C_L C_B^2}{2}.
\end{align}
By further setting the constant step-size as
\begin{equation} \label{eq:prthm165}
\begin{split}
\alpha \!=\! \sqrt{\frac{2\left( \bar{C} (\ccalH_0) - \bar{C} (\ccalH^*)\right)}{T C_L C_B^2 }}
\end{split}
\end{equation}
and substituting it into \eqref{eq:prthm16}, we have
\begin{equation} \label{eq:prthm17}
\begin{split}
&\min_t \mathbb{E}[\| \nabla_\ccalH \bar{C}(\ccalH_t) \|^2] \le \frac{C}{\sqrt{T}}
\end{split}
\end{equation}
with constant $C\!=\! \sqrt{2\!\left( \bar{C} (\ccalH_0) - \bar{C} (\ccalH^*)\right)\!C_L}C_B$. Therefore, the bound decreases to zero with the rate $\mathcal{O}(1/\sqrt{T})$. This completes the proof.
\end{proof}
